Local Vertex Colouring Graph Neural Networks

In recent years, there has been a significant amount of research focused on expanding the expressivity of Graph Neural Networks (GNNs) beyond the Weisfeiler-Lehman (1-WL) framework. While many of these studies have yielded advancements in expressivity, they have frequently come at the expense of decreased efficiency or have been restricted to specific types of graphs. In this study, we investigate the expressivity of GNNs from the perspective of graph search. Specifically, we propose a new vertex colouring scheme and demonstrate that classical search algorithms can efficiently compute graph representations that extend beyond the 1-WL. We show the colouring scheme inherits useful properties from graph search that can help solve problems like graph biconnectivity. Furthermore, we show that under certain conditions, the expressivity of GNNs increases hierarchically with the radius of the search neighbourhood. To further investigate the proposed scheme, we develop a new type of GNN based on two search strategies, breadth-first search and depth-first search, highlighting the graph properties they can capture on top of 1-WL. Our code is available at https://github.com/seanli3/lvc.

==> sections/Qing-notes.tex <==
\clearpage
\section{Notes from Qing}

Let $G=(V,E)$ be an undirected graph and $S(v)$ be a search on the nodes in the  neighbourhood $N_{\delta}(v)$ on $G$, starting from a vertex $v\in V$. We denote the set of tree edges in the search by $S_{dfs}(v)$ as $tree(E)$, the set of back edges as $back(E)$, and the set of cross edges as $cross(E)$ (definitions come later). A \emph{beeline path} $(w_0,w_1,\dots,w_k)$ in $N_{\delta}(v)$ is defined as a path satisfying: $w_0=v$, $hop(w_{i-1})+1=hop(w_{i})$ and $w_i\in N_{\delta}(v)$ for $i=1,\dots, k$.

For each $v\in V$, we associate it with a hop-aware neighborhood subgraph, defined as $G_v=(V_v, E_v, \pi)$ where $V_v=N_{\delta}(v)\cup \{v\}$, $E_v=\{(u,u')\in E|u,u'\in N_{\delta}(v)\}$, and $\pi: V\times V\rightarrow\mathbb{N}$ assigns a hop number to each node in this subgraph such that $\pi(v,u)=d_{vu}$ and we consider $d_{vv}=0$.

\begin{itemize}
\item \emph{Breadth-first Coloring} (BFC): \\ Starting from a source vertex $v$, BFC traverses on its hop-aware neighbourhood subgraph $G_v$ in a breadth-first searching manner and colours each node along the traversal. More specifically,  BFC colours the nodes in the neighbourhood $N_{\delta}(v)$ of a source vertex $v$ at increasing distances from the immediate neighbors of $v$ to the farthest neighbors of $v$, as defined below:

\begin{equation}
\label{eqn:bfs_lvc_forward}
    \lambda^{l+1}_v(w):= \phi\Bigl(\lambda^{l}_v(w), \psi\bigl(\lambda^{l}_{tree}(w), \lambda_{back}^{l}(w), \lambda_{cross}^{l}\bigr)\Bigr)
\end{equation}

($\lambda_{tree}$, $\lambda_{back}$, and $\lambda_{cross}$ need to be defined later)

For BFC, the following property holds.
\begin{lemma}
 For any beeline path $(w_0,w_1,\dots,w_k)$ in $N_{\delta}(v)$, $w_{i-1}$ is colored \emph{before} $w_i$ for $i=1,\dots, k$.   
\end{lemma}



\item  \emph{Depth-first Coloring} (DFC): \\
Starting from a source vertex $v$, DFC traverses on its hop-aware neighborhood subgraph $G_v$ in a depth-first searching manner and colors each node when it traverses reversely back from the node. More specifically, DFC traverses as depth as possible and colors a node when the node has all child nodes at a deeper level visited (the definition of the traversal needs to be formalised later). When coloring a node, the same method as BFC can be defined:

\begin{equation}
\label{eqn:bfs_lvc_forward}
    \lambda^{l+1}_v(w):= \phi\Bigl(\lambda^{l}_v(w), \psi\bigl(\lambda^{l}_{tree}(w), \lambda_{back}^{l}(w), \lambda_{cross}^{l}\bigr)\Bigr)
\end{equation}

For DFC, the following property can hold.
\begin{lemma}
For any beeline path $(w_0,w_1,\dots,w_k)$ in $N_{\delta}(v)$, $w_{i-1}$ is colored \emph{after} $w_i$ for $i=1,\dots, k$.
\end{lemma}

For DFC, we can show that it can be applied for cycle detection and finding articulation points.

\end{itemize}

